SelfPose: 3D Egocentric Pose Estimation from a Headset Mounted Camera

We present a solution to egocentric 3D body pose estimation from monocular images captured from downward looking fish-eye cameras installed on the rim of a head mounted VR device. This unusual viewpoint leads to images with unique visual appearance, with severe self-occlusions and perspective distortions that result in drastic differences in resolution between lower and upper body. We propose an encoder-decoder architecture with a novel multi-branch decoder designed to account for the varying uncertainty in 2D predictions. The quantitative evaluation, on synthetic and real-world datasets, shows that our strategy leads to substantial improvements in accuracy over state of the art egocentric approaches. To tackle the lack of labelled data we also introduced a large photo-realistic synthetic dataset. xR-EgoPose offers high quality renderings of people with diverse skintones, body shapes and clothing, performing a range of actions. Our experiments show that the high variability in our new synthetic training corpus leads to good generalization to real world footage and to state of theart results on real world datasets with ground truth. Moreover, an evaluation on the Human3.6M benchmark shows that the performance of our method is on par with top performing approaches on the more classic problem of 3D human pose from a third person viewpoint.

==> sections/challenges.tex <==
%Egocentric 3D human pose estimation differs considerably from the more
%standard scenario of outside-in looking cameras.
%%% HB Comment: these are full paragraph items, so we write each item
%%% starting with capital letters.
%%\begin{itemize}
%%\item 
%%Standard approaches to 
%%% \item Front-facing cameras capture bodies with little
%%%   self-occlusion. On the contrary, form the egocentric perspective the
%%%   lower-body areas are self-occluded most of the time making the
%%%   problem much harder to solve and requiring a strong inference
%%%   machine to deal with the problem. An example of the severity of this
%%%   problem is shown as white areas in the top row of
%%%   Fig.~\ref{fig:perspective}.
%%% \item Standard approaches usually use pinhole camera models with
%%%   relatively low lens distortion. The subject usually also stands at a
%%%   relatively large distance allowing to even assume orthogonal
%%%   projection. Instead, egocentric approaches use wide or fish-eye
%%%   lenses to capture as much of the body as possible to increase the
%%%   observability of the body parts (see bottom row of Figure
%%%   \ref{fig:perspective}).
%%\end{itemize}



% Figure~\ref{fig:perspective} shows several poses captured from both
% an external and an egocentric point of view. This allows us to
% understand why this is such a hard problem. The highlighted areas on
% the character represent the part on the mesh that visible from the
% egocentric camera, mounted on the headset. It is clear that for most
% of the poses there is a large amount of self-occlusion, mainly on
% the lower body due to the chest. This is one of the main challenges
% of this specific task. Another problem of solving human pose
% estimation from an egocentric point of view is about the resolution
% of the different parts of the body. As it is possible to see from
% the figure, the amount of pixels used to represent the feet is way
% less for example compared to the amount of pixels for the hands.

%% Images acquired from \textit{front facing cameras} exhibit
%% mild self-occlusions, uniform pixel density for all body parts and
%% negligible perspective effects (close to orthographic conditions). In
%% contrast, images captured from egocentric setups have severe
%% self-occlusions, extreme perspective effects, due to the use of
%% wide-angle lenses, and vastly different pixel density for the upper
%% and lower body. 


\textcolor{red}{F: I put this section in the Introduction, probably we can remove this section. The Challenges should be part of the motivation of the work, and goes to the introduction.  },

Fig.~\ref{fig:perspective} provides a visualization of the unique
visual appearance of our HMD egocentric setup --- the top row shows
which body parts would become self-occluded from an egocentric
viewpoint. The continuous graduation from bright red to dark green 
encodes the increasing pixel resolution for the corresponding colored area.
%% and dark green indicates highest and bright red lowest spatial
%%resolution. 
This unusual visual appearance calls both for a new
approach and a new training corpus. Our paper tackles both. Our new
neural network architecture encodes the
difference in uncertainty between upper and lower body joints caused
by the varying resolution, extreme perspective effects and
self-occlusions. On the other hand, our new large-scale synthetic
training set --- {\boldmath $x$}R-EgoPose --- contains $383$K images
rendered from a novel viewpoint: a fish-eye camera mounted on a VR
display. It has quite superior levels of photo-realism in contrast with
the only other existing monocular egocentric
dataset~\cite{xu2019mo2cap2} (see Fig.~\ref{fig:comparison_mo2cap2}
for a side to side comparison), and large variability in the data. To
enable quantitative evaluations on real world images, we contribute
{\boldmath $x$}R-EgoPose$^\text{R}$, a smaller scale real-world
dataset acquired with a lightweight setup -- a real fish-eye camera
mounted on a VR display -- with ground truth 3D pose annotations. Our
extensive experimental evaluations show that our new approach
outperforms the current state of the art in monocular egocentric 3D
pose estimation~\cite{xu2019mo2cap2} both on synthetic and real-world
datasets.
